Systematic Evaluation of Initial States and Exploration-Exploitation Strategies in PID Auto-Tuning: A Framework-Driven Approach Applied on Mobile Robots

PID controllers are widely used in control systems because of their simplicity and effectiveness. Although advanced optimization techniques such as Bayesian Optimization and Differential Evolution have been applied to address the challenges of automatic tuning of PID controllers, the influence of initial system states on convergence and the balance between exploration and exploitation remains underexplored. Moreover, experimenting the influence directly on real cyber-physical systems such as mobile robots is crucial for deriving realistic insights. In the present paper, a novel framework is introduced to evaluate the impact of systematically varying these factors on the PID auto-tuning processes that utilize Bayesian Optimization and Differential Evolution. Testing was conducted on two distinct PID-controlled robotic platforms, an omnidirectional robot and a differential drive mobile robot, to assess the effects on convergence rate, settling time, rise time, and overshoot percentage. As a result, the experimental outcomes yield evidence on the effects of the systematic variations, thereby providing an empirical basis for future research studies in the field.

==> Sections/Evaluation.tex <==
\textcolor{orange}{Add description about the steady stata error (what causes it? why in some cases its high/low)}
% In this section, we evaluate our study using a case study from the mobile robotics domain, focusing on a custom-designed DDMR constructed specifically for this research. The study involves auto-tuning of a PID controller , which is a fundamental feedback control mechanism, widely used in control systems engineering for its simplicity and effectiveness in managing system dynamics, as mentioned in Section \ref{sec:introduction}. 
% This evaluation aims to assess the ability of BO and DE to escape local optima and converge in DDMR, examine the impact of various initial PID gain values (Section~\ref{sec:methodology}) on convergence rates, speed and settling times, and explore the effects of three distinct search configurations on optimization outcomes.

This section presents the evaluation results obtained by applying the Framework to two types of robots: the DDRM and the Omnidirectional robots. The analysis is organized around three research questions. Specifically, it aims to assess the ability of BO and DE to escape local optima and achieve convergence under different initial PID gain values, and to investigate the impact of three distinct EECs on the optimization outcomes  (as detailed in Section~\ref{sec:methodology}).

\textbf{RQ1 (Convergence of BO and DE)}\label{sssec:evaluation-rq1} \textit{What is the propensity of BO and DE optimization algorithms to end up in local optima?}  This research question assesses how effectively BO and DE can escape local optima by analyzing their performance over multiple trials. A total of 120 trials were conducted, with both algorithms initialized using identical EEC and initial state in each trial. For a trial to be considered successfully converged, the optimizer must reach the target -defined as achieving a settling time of 2500~ms or less- while satisfying the constraints outlined in Section~\ref{ssec:experimental_setting} and doing so within a maximum of 150 iterations. If these conditions are met, the trial is deemed successful; otherwise, the optimizer is considered trapped in a local optimum.

\textbf{RQ2 (Initial State Impact)} \textit{What is the impact of the initial state on the optimizers' convergence speed, settling time, and optimal gain values?}  
This research question explores how various initial states affect the performance of the optimizers under a balanced exploration-exploitation setting (EEC 0, as defined in Table~\ref{tab:configs-def}). EEC 0 was chosen because it provides an unbiased environment that equally emphasizes exploration and exploitation. This balanced setting allows us to directly observe the influence of different initial states on convergence speed, settling time, and the determination of optimal gain values without the confounding effects of extreme biases.

\textbf{RQ3 (Search Configurations Impact)} \textit{How do different configurations of the optimizers influence their final convergence behavior, including the likelihood of getting trapped in local optima, convergence speed, settling time, and the determination of optimal gain values?}  
This research question investigates the effects of three distinct EEC, as outlined in Table~\ref{tab:configs-def}, across two initial states. The goal is to evaluate how these varying configurations affect the optimizers’ overall performance, specifically their ability to converge, robustness against local optima, convergence speed, settling time, and the process of determining optimal gain values.


% \subsection{Study Subject}
% Our study subject involves a Differential Drive Mobile Robot (DDMR). The robot contains two front caster wheels and two pairs of JS5230 aluminum-silicon wheel sets\cite{js5230Jsumo}, each with a diameter of 52 mm and a width of 30 mm . It is also equipped with an H-Bridge L298-N motor driver \cite{HBridgeL298}, which provides precise control over motor direction and speed. The robot utilizes Titan DC Gear~\cite{MotorTitanDCGearhead} head Motors with a 12V supply and 500 RPM speed. These motors are known for their robustness and high torque, making them suitable for precise control applications. For real-time angular data acquisition, the Nicla Sense ME \cite{BoschSensortecNiclaSense} was selected due to its advanced sensor fusion capabilities. This sensor integrates data from a 3-axis accelerometer, 3-axis gyroscope, magnetometer, and environmental sensor, ensuring highly accurate and reliable angle measurements. The robot's chassis was custom-designed and 3D-printed, offering a lightweight yet sturdy framework that supports rapid prototyping and design flexibility. The processing unit, which runs the program, is Jetson Nano \cite{jetsonNano}. Jetson Nano is equipped with an NVIDIA Maxwell GPU and a quad-core ARM Cortex A57 CPU, delivering 472 GFLOPs of computational power.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{Images/merged.jpg}
%     \caption{Photos for our study subject robot}
%     \label{fig:robot}
% \end{figure}
%% The real photo of the robot is hidden. Not referenced any more

% \textbf{Kinematics Model:}

% DDMRs use a common drive mechanism consisting of two independently driven wheels mounted on the same axis. This configuration allows the robot to vary its trajectory by adjusting the velocities of the left and right wheels, denoted as $V_l$ and $V_r$, respectively \cite{kinematics}.

% \begin{enumerate}
%     \item \textbf{Instantaneous Center of Curvature (ICC)}
% The robot's motion is characterized by the Instantaneous Center of Curvature (ICC), which lies along the axis between the wheels. The robot's rotation rate $\omega$ about the ICC is identical for both wheels, leading to the kinematic Equations \ref{eq:ICC1} and \ref{eq:ICC2}.

% \begin{equation}\label{eq:ICC1}
% \omega (R + \frac{l}{2}) = V_r,
% \end{equation}

% \begin{equation}\label{eq:ICC2}
% \omega (R - \frac{l}{2}) = V_l,
% \end{equation}

% where:
% \begin{itemize}
%     \item $l$ is the distance between the centers of the two wheels,
%     \item $R$ is the signed distance from the ICC to the midpoint between the wheels,
%     \item $V_r$ and $V_l$ are the linear velocities of the right and left wheels, respectively.
% \end{itemize}

% The ICC and the rate of rotation $\omega$ can be determined using Equation \ref{eq:ICC3}.

% \begin{equation}\label{eq:ICC3}
% R = \frac{l}{2} \frac{V_l + V_r}{V_r - V_l}, \quad \omega = \frac{V_r - V_l}{l}.
% \end{equation}

%     \item \textbf{Special Cases}

% The differential drive configuration exhibits three notable cases:
% \begin{enumerate}
%     \item If $V_l = V_r$, the robot moves in a straight line with no rotation ($R \to \infty$ and $\omega = 0$).
%     \item If $V_l = -V_r$, the robot rotates in place about the midpoint between the wheels ($R = 0$).
%     \item If the velocity of one wheel is zero (e.g., $V_l = 0$), the robot rotates about the stationary wheel ($R = -\frac{l}{2}$).
% \end{enumerate}


%     \item \textbf{Forward Kinematics}
% Assuming the robot is at a position $(x, y)$ with an orientation $\theta$ relative to the X-axis, the robot's pose after time $\delta t$ can be determined using the transformation matrix based on the ICC coordinates, as given in Equation \ref{eq:forward-kinmatics-matrix}.

% \begin{equation}\label{eq:forward-kinmatics-matrix}
% \resizebox{.5\hsize}{!}{$
% \begin{bmatrix}
% x' \\
% y' \\
% \theta'
% \end{bmatrix}
% =
% \begin{bmatrix}
% \cos(\omega \delta t) & -\sin(\omega \delta t) & 0 \\
% \sin(\omega \delta t) & \cos(\omega \delta t) & 0 \\
% 0 & 0 & 1
% \end{bmatrix}
% \begin{bmatrix}
% x - ICC_x \\
% y - ICC_y \\
% \theta
% \end{bmatrix}
% +
% \begin{bmatrix}
% ICC_x \\
% ICC_y \\
% \omega \delta t
% \end{bmatrix},
% $}
% \end{equation}

% where $(ICC_x, ICC_y)$ represents the location of the ICC. This model describes the movement of the robot as it rotates around its ICC with angular velocity $\omega$.
% \end{enumerate}
%% TODO (Already DONE): Add kinematics model - Ref: https://www.cs.columbia.edu/~allen/F19/NOTES/icckinematics.pdf

\subsection{Experimental Settings} 
\label{ssec:experimental_setting}
We configured the DE and BO algorithms based on the parameter setting outlined in Table \ref{tab:configs-def}.

\begin{enumerate}
    \item Differential Evolution Configurations

The DE algorithm is tuned using different combinations of mutation and crossover rates to explore diverse search strategies:
\begin{itemize}
    \item \textbf{EEC 0} employs a balanced exploration-exploitation approach with a mutation rate of 60\% and a crossover rate of 60\%, suitable for a moderate exploration of the solution space.
    \item \textbf{EEC 1} emphasized exploration by setting a higher mutation rate (80\%) and a lower crossover rate (30\%), aiming to increase diversity and reduce premature convergence.
    \item \textbf{EEC 2} focuses on exploitation with a mutation rate of 50\% and a high crossover rate of 90\%, enhancing the refinement of solutions by leveraging known high quality solutions.
\end{itemize}

The remaining parameters for the DE algorithm are set as follows: both the relative tolerance (\textit{tol}) and the absolute tolerance (\textit{atol}) for convergence were set to 0.0, indicating a strict convergence criterion. The optimization process utilized a single worker, reflecting the constraint of operating on a single robot, thus precluding the use of multiple parallel agents. No post-optimization polishing is applied to the best population member, and the population size is configured to 15. The \textit{"rand1bin"} strategy was selected, characterized its use of a randomly chosen vector for mutation and binomial crossover to create a new candidate solutions.

\item Bayesian Optimization Configurations
For the BO, the configurations adjust the expected improvement parameter ($\xi$) to modulate the balance between exploration and exploitation:
\begin{itemize}
    \item \textbf{EEC 0} sets $\xi$ to 0.1, encouraging a balanced approach.
    \item \textbf{EEC 1} increases $\xi$ to 0.2, promoting exploratory behavior by seeking potentially high-reward regions.
    \item \textbf{EEC 2} reduces $\xi$ to 0.01, heavily favoring exploitation by focusing on regions with already promising results.
\end{itemize}

% No transformation is applied to the parameters bounds during the optimization process. Duplicate sampling of points were not permitted, as the PID control for the DDMR operates in a low-noise environment where repeated evaluation of the same point would yield consistent results.
\end{enumerate}

The PID gains ($K_p$, $K_i$, $K_d$) are bounded within the optimization process as follows: $K_p$ (1 to 25), $K_i$ (0 to 1), and $K_d$ (0 to 1), defining the search space for the optimizers. The constraints are a maximum overshoot percentage of 30\% and a maximum rise time of 1000 ms

The trials were constrained to a maximum of 150 iterations to achieve successful convergence. The experiment duration was set to 5000 ms with a sampling interval of 100 ms for the DDRM, and 10000 ms for the Onmidirectional. This ensures equal weighting of each run by recording values at every 100 ms interval to avoid bias. The set point for all trials was fixed at 90\textdegree, allowing a maximum overshoot of up to 120\textdegree. The optimizer objective was to achieve a settling time of 2500 ms or less. Each optimizer was required to run across the 6 initial states described in Section \ref{ssec:init_states} for each of the 3 different configurations, resulting in a total of 36 trials, the average time for a converged trial is 888 seconds (14 minutes and 48 seconds), and the total time for all the converged trials was 459 minutes (7 hours and 39 minutes).
The trials were carried out using Python and C++ programming languages. We utilized the SciPy \cite{2020SciPy} and Bayesian-Optimization \cite{BO-library} libraries to execute the optimization algorithms. For data analysis and visualization, we employed Pandas \cite{pandas}, Matplotlib \cite{matplotlib},  and Seaborn \cite{seaborn}. Communication with the microcontroller was done using PySerial \cite{pyserial}. The C++ package "Arduino BHY2" \cite{Arduino_BHY2} was utilized to extract sensor fusion data from the Nicla Sense ME. After obtaining the robot's heading (yaw angle), the error is calculated and subsequently fed into the PID control system as mention in Section \ref{sec:introduction}.

%We configure DE and BO using the parameters in Table~\ref{tab:configs-def} \textcolor{blue}{DE and BO search configuration params (mutation and crossover values) should be detailed here. please create a table for DE with all the search parameters (pop size, mutation/cross rate, selection method and rates number of generations, constants values)}

%\textcolor{blue}{describe the inputs and outputs of your experiment scripts, how many runs and what the final result you obtain from the experiment}.


\begin{table*}[t]
    \centering
    \caption{DE and BO optimizers configurations}
    \label{tab:configs-def}
    \begin{tabularx}{\textwidth}{|c|X|X|X|} \hline 
         Configuration ID & Representation & DE - config parameters & BO - config parameters \\ \hline 
         0 & Balanced Exploration-Exploitation optimization & Mutation Rate: 60\%, Crossover Rate: 60\% & Expected Improvement $\xi$: 0.1 \\ \hline 
         1 & Exploration-Focused optimization & Mutation Rate: 80\%, Crossover Rate: 30\% & Expected Improvement $\xi$: 0.2 \\ \hline 
         2 & Exploitation-Focused optimization & Mutation Rate: 50\%, Crossover Rate: 90\% & Expected Improvement $\xi$: 0.01 \\ \hline
    \end{tabularx} 
\end{table*}

\subsection{Results}

\textbf{RQ1.} This research question evaluates the average convergence rates of BO and DE based on all trials conducted, which included three configurations with six trials each. The average convergence rate reflects how often each optimizer successfully reached the objective settling time value without getting trapped in local optima across all these trials. Figure \ref{fig:rq1-avg-conv-rate} visualize the results. BO achieved an average convergence rate of 77.8\%, showing some vulnerability to local optima, where it could not minimize the settling time to 2500 ms or less; due to not exploring enough various gain values within the search space. In contrast, DE achieved a perfect average convergence rate of 100\% across all trials, consistently avoiding local traps.

These results demonstrate that DE is more reliable than BO in terms of convergence, maintaining perfect performance across all configurations and initial settings. While BO can still be effective, its tendency to get trapped in local optima indicates that it may need further tuning to match DE’s robustness and do broader exploration.

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{Images/rq1-chart.png}
    \caption{Average convergence rate for BO and DE, across all trials}
    \label{fig:rq1-avg-conv-rate}
\end{figure}
%Figure \ref{fig:config-convergence-rate} further breaks down the convergence rates by configuration. For Configuration IDs 1 and 2, BO experienced a convergence rate of 66.67\%, indicating a notable difficulty in these specific settings. The data suggest that BO has a higher likelihood of getting trapped in local optima, particularly in more complex or challenging configurations. In contrast, DE maintained a convergence rate of 100\% in all configurations, demonstrating a strong ability to avoid local optimizations and reach global solutions.
\iffalse
\begin{table}[t]
  \centering
  \caption{Optimizer Identifier (Opt ID); Configuration Identifier (Config ID); Number of Trials Trapped in Local Optima (Trapped) Across 6 Trials; Convergence Percentage (Conv~\%) for Each Configuration; and Average Convergence Percentage (Conv~\%) Across Three Configurations for Each Optimization Technique, for our Study Subject, Based on the Parameters in Table~\ref{tab:configs-def}}
  \label{table:config-convergence-rate}
  \begin{tabular}{|c|c|c|c|c|}
  \hline
    \textbf{Opt ID}& \textbf{Config ID}& \textbf{Trapped}& \textbf{Conv~\%}& \textbf{Avg Conv~\%}\\
    \hline
    \multirow{3}{*}{BO} & 0& 0&  100&\multirow{3}{*}{77.8}\\
    & 1& 2& 66.67 &\\
    & 2& 2& 66.67 &\\
    \hline
    \multirow{3}{*}{DE} & 0& 0&  100&\multirow{3}{*}{100}\\
    & 1& 0& 100 &\\
    & 2& 0 & 100&\\
    \hline
  \end{tabular}
\end{table}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Images/convergence_and_trapped_trials.png}
    \caption{Convergence and Trapped Trials by Configuration for BO and DE}
    \label{fig:config-convergence-rate}
\end{figure}
\fi
%This analysis also opens avenues for the next research questions, as to thoroughly investigate the impact of initial states and search configurations on the performance of these algorithms in a study that leverage the strengths and weaknesses of both methods.
% add a smooth intro to initial state (RQ2)

%\begin{table*}[t]
%  \centering
%  \caption{Overall Convergence Rate}
%  \label{table:overall-convergence-rate}
%  \begin{tabular}{|c|c|c|c|}
%  \hline
%    Optimizer& \# Trapped& \# Trials& Convergence (\%)\\
%    \hline
%    Bayesian Optimizer& 4& 18& 77.78\\
%    Differential Evolution& 0& 18& 100\\
%    \hline
%  \end{tabular}
%\end{table*}



%\subsubsection{Bayesian Optimizer Trapping Propensity} \label{rq1-bo}
%\subsubsection{Differential Evolution Trapping Propensity} \label{rq1-de}
%\subsubsection{Optimizers Comparison Trapping Propensity} \label{rq1-com}
% \begin{framed}
% \end{framed}


%\begin{tcolorbox}[colback=gray!10!white,colframe=black!75!black]
%The answer to RQ1 is that  
%\end{tcolorbox}

\begin{tcolorbox}[colback=gray!10!white,colframe=black!75!black] 
The answer to RQ1 is that DE consistently outperforms BO in escaping local optima, achieving a 100\% convergence rate in all configurations and initial states. In contrast, BO reaches a convergence rate of 77.78\%, highlighting DE's superior ability to avoid suboptimal regions.
\end{tcolorbox}


\textbf{RQ2.} Table \ref{table:balanced-exploration-exploitation} summarizes the trial results of BO and DE under a balanced exploration-exploitation configuration. Particularly, it presents for each initial state the performance metrics for both optimizers. The metrics are  convergence time,  number of iterations, settling time, steady-state error, and PID gain values ($K_p$, $K_i$, $K_d$) that led to the desired objective settling time value -or-less- and achieved overshoot percentage and raise time values within the constraints mentioned in \ref{ssec:experimental_setting}. Note that to answer this question, we decided to focus on the balanced exploration-exploitation configuration. However, the performance results of the optimizers under the other two configurations -described in Section \ref{ssec:init_states}, are available with further details via the shared annex on Zenodo ~\cite{PID-Tuning-for-Motion-Optimization} on trial\_results page.
%\textcolor{red}{Add Zenodo here}

Figure \ref{fig:iterations-time-balanced} shows the time and number of iterations required by DE and BO to complete the trials for each initial state. The results highlight a clear difference in time efficiency between the two optimizers. BO generally finds solutions faster than DE across most initial states; for example, BO completed the task in 44 seconds compared to DE’s 350 seconds in initial state 0. However, in initial states 3 and 4, BO took significantly longer, at 7396 and 4358 seconds, respectively, compared to DE’s 581 and 146 seconds. This indicates that BO’s performance can be highly sensitive to the initial values used to build the initial surrogate model, leading to extended exploration times in some cases. Further, the number of iterations required for convergence also varies significantly between the two methods. BO consistently converges in fewer iterations than DE. In initial state 0, for instance, BO reached convergence in just 3 iterations, whereas DE needed 31 iterations. This indicates that although BO sometimes requires more computational time (as seen in initial states 3 and 4), it is capable of finding solutions in fewer steps, which can be an advantage when iteration costs are high or when rapid convergence is desired.

Figure~\ref{fig:settling_time_kdes} presents kernel density estimation (KDE) plots comparing the minimum settling times achieved by DE and BO across all trials. In the case of balanced exploration-exploitation configuration (left plot), BO shows a slightly lower median settling time than DE, indicating its effectiveness in finding optimal PID parameters under this configuration. Similarly, Figure~\ref{fig:steady_state_error_kdes} displays KDE plots for steady-state errors, where it exhibits a narrower distribution for steady-state errors achieved by BO besides a median error closer to zero, compared to DE's broader and less peaked KDE . This demonstrates BO’s greater effectiveness in minimizing steady-state error under the balanced exploration-exploitation configuration.


Figure \ref{fig:gain-balanced} shows the PID gain values for BO and DE for the 6 initial states. The three subplots represent the proportional ($K_p$), integral ($K_i$) and derivative ($K_d$) gains, respectively.  Each gain is plotted against various initial states, comparing the values obtained by BO (blue) and DE (red). As shown, DE consistently produces higher proportional gains $K_p$ than BO. For example, in initial state 4, DE's $K_p$ is 20.15, whereas BO's is 4.93, but in initial state 5, BO's $K_p$ is slightly higher than DE's. This variability suggests that both algorithms dynamically adapt their gain selection strategies to the characteristics of the optimization landscape. Furthermore, DE often adjusts its integral gain $K_i$ more aggressively to reduce steady-state error, while DE appears to favor higher derivative gains $K_d$ in certain cases, possibly to control overshooting and enhance system damping. These differences reflect each algorithm's approach to balancing convergence speed with stability, indicating that their performances vary depending on the initial conditions.


\begin{table*}[t]
  \centering
  \caption{Balanced Exploration-Exploitation}
  \label{table:balanced-exploration-exploitation}
  \resizebox{\textwidth}{!}{ % Resize the table to fit the width of the page
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
    \hline
      Initial State & Optimizer & Time (s) & \# Iterations & Settling Time (ms) & Steady State Error (deg) & $K_p$ & $K_i$ & $K_d$ \\
      \hline
      \multirow{2}{*}{0} & BO & 44 & 3 & 2400 & 2.44 & 10.907680 & 0.330117 & 0.127006 \\
      & DE & 350 & 31 & 2400 & 1.55 & 16.0 & 0.0 & 0.96426 \\ 
      \hline 
      \multirow{2}{*}{1} & BO & 73 & 5 & 1300 & 0.19 & 18.249986 & 0.740096 & 0.708124 \\
      & DE & 1452 & 126 & 1800 & 3.31 & 23.703049 & 0.261754 & 0.971221 \\ 
      \hline 
      \multirow{2}{*}{2} & BO & 115 & 8 & 1600 & -0.53 & 6.788276 & 0.049277 & 0.409347 \\
      & DE & 364 & 36 & 1400 & 2.09 & 6.432 & 0.078199 & 0.782228 \\ 
      \hline
      \multirow{2}{*}{3} & BO & 7396 & 121 & 1100 & -0.17 & 17.801146 & 0.670552 & 0.476415 \\
      & DE & 581 & 46 & 1800 & 1.4 & 18.723926 & 0.162630 & 0.471297 \\ 
      \hline
      \multirow{2}{*}{4} & BO & 4358 & 115 & 1300 & -0.16 & 4.930022 & 0.085849 & 0.263449 \\
      & DE & 146 & 11 & 2500 & 17.35 & 20.154038 & 0.07 & 0.892 \\ 
      \hline
      \multirow{2}{*}{5} & BO & 570 & 31 & 1800 & 1.65 & 13.058583 & 0.080072 & 0.188088 \\
      & DE & 436 & 41 & 1600 & 4.27 & 9.517405 & 0.078128 & 0.325520 \\ 
      \hline
    \end{tabular}
  }
\end{table*}




\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{Images/rq2_iterations_time_balanced.png}
    \caption{Iteration and Time By Initial State and Optimizer}
    \label{fig:iterations-time-balanced}
%\end{figure}
%\begin{figure}
%    \centering
    \includegraphics[width=0.75\linewidth]{Images/rq2_pid_gains_scatter_balanced.png}
    \caption{PID Gain Values by Initial State and Optimizer}
    \label{fig:gain-balanced}
\end{figure}



\begin{tcolorbox}[colback=gray!10!white,colframe=black!75!black] 
The answer to RQ2 is that the initial state significantly impacts the optimizer performance. BO often achieves lower steady-state errors and settling times when it is compared with DE, but it struggles with local optima for some initial states. DE consistently provides reliable convergence across all initial states, showing high adaptability, although with slightly higher steady-state-errors compared to BO.
%the initial state has a significant impact on the optimization performance of both BO and DE. 

%\textbf{Finding 1:} On average, BO converges faster and requires fewer iterations, but its performance decreases when operating with lower $K_d$ values%inducting more efficient exploration, 

%\textbf{Finding 2:} On average, DE is less efficient than BO but achieves higher proportional and derivative gains.

%This behavior reflects each optimizer's distinct strategies in balancing speed and stability, influenced by the initial states.
\end{tcolorbox}

\textbf{RQ3} The convergence behavior of BO and DE is significantly influenced by different configurations. BO converges faster in terms of iterations but is more susceptible to local optima, as discussed in Section \ref{sssec:evaluation-rq1}. This issue is particularly clear in complex scenarios where BO sometimes fails to converge. DE, though slower and requiring more iterations, shows greater resilience against local optima, often finding solutions when BO struggles.  These findings can be seen in the obtained results in Tables \ref{table:exploration-focused} and \ref{table:exploitation-focused}). In the Balanced Exploration-Exploitation configuration, the results are shown in Table \ref{table:balanced-exploration-exploitation}. BO’s aggressive exploitation strategy enables rapid convergence but can lead to longer computational times due to over-exploitation of certain search areas. DE’s convergence speed varies by configuration, generally requiring more time due to its broader search and refinement process, which helps avoid local optima but slows convergence, as seen in exploration-focused results, presented in Table \ref{table:exploration-focused}. BO typically achieves shorter reset times across most configurations, as shown in the KDE Figure \ref{fig:settling_time_kdes}. Its configurations are optimized for fast responses, focusing on efficient exploitation of promising regions. In contrast, DE shows greater variability and longer settling times due to its extensive exploration phases, which are less tuned for rapid responses, especially in exploitation-focused scenarios. The configuration's influence is also reflected in the determination of optimal gain values ($K_p$, $K_i$, $K_d$). BO produces more stable and precise gains, resulting in lower steady-state errors and consistent performance, as shown in Figure \ref{fig:steady_state_error_kdes}. DE, however, has higher variability in its gain values, reflecting a broader search space that occasionally compromises tuning precision. This variability highlights a trade-off in DE between exploring diverse solutions and achieving efficient control parameter optimization leading to low steady-state-error.

\begin{tcolorbox}[colback=gray!10!white,colframe=black!75!black] 
The answer of RQ3 is that different configurations affect BO and DE’s convergence behavior significantly. BO offers faster convergence and shorter settling times, but is more prone to local optima. DE explores broadly, reducing the risk of local traps but converges slower with higher variability. BO finds more precise gains, while DE balances exploration and robustness.
\end{tcolorbox}


 


\begin{table*}[t]
  \centering
  \caption{Exploration Focused}
  \label{table:exploration-focused}
  \resizebox{\textwidth}{!}{ % Resize the table to fit the width of the page
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \hline
      Initial State & Optimizer & Time (s) & \# Iterations & Settling Time (ms) & Steady State Error (deg) & $K_p$ & $K_i$ & $K_d$ \\ \hline
      \multirow{2}{*}{4} & BO & 330 & 22 & 1700 & -2.41 & 6.63 & 0.020 & 0.66 \\
      & DE & 420 & 31 & 2400 & 1.08 & 15.69 & 0.082 & 0.71 \\ \hline
      \multirow{2}{*}{5} & BO & didn't converge & 150 & - & - & - & - & - \\
      & DE & 1363 & 111 & 2500 & 4.45 & 18.54 & 0.33 & 0.82 \\ \hline
    \end{tabular}
  }
\end{table*}


\begin{table*}[t]
  \centering
  \caption{Exploitation Focused}
  \label{table:exploitation-focused}
  \resizebox{\textwidth}{!}{ % Resize the table to fit the width of the page
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \hline
      Initial State & Optimizer & Time (s) & \# Iterations & Settling Time (ms) & Steady State Error (deg) & $K_p$ & $K_i$ & $K_d$ \\ \hline
      \multirow{2}{*}{4} & BO & 242 & 17 & 2100 & 3.61 & 12.24& 0.17& 0.76\\
      & DE & 218 & 16 & 1600 & 4.46 & 4.20& 0.001 & 1.0 \\ \hline
      \multirow{2}{*}{5} & BO & didn't converge & 150 & - & - & - & - & - \\
      & DE & 1276 & 91 & 2400 & 6.57 & 12.91& 0.0033& 0.091\\ \hline
    \end{tabular}
  }
\end{table*}





\begin{figure}[htb!]
    \centering
        \includegraphics[width=\linewidth]{Images/settling_time_low_res.png}
        \caption{Settling Time KDE}
        \label{fig:settling_time_kdes}
\end{figure}
%As shown in figure \ref{fig:settling_time_kdes}, for the balanced exploration-exploitation configuration, the KDE plot (left) shows a notable overlap between the two algorithms, with the BO demonstrating a slightly lower median settling time than DE. This suggests that the BO more effectively identifies optimal PID parameters when a balanced between exploration and exploitation is maintained. In the exploration-focused configuration (middle plot), the BO presents a narrower and more peaked distribution, indicating a higher consistency and generally shorter settling times compared to DE, which displays a broader distribution skewed toward longer settling times. In the exploitation-focused configuration (right plot), the distribution curves of both algorithms are more aligned, with the BO still maintaining a marginal advantage in achieving lower settling times. Overall, these findings suggest that while both algorithms can be effective under different strategies, the BO consistently delivers faster convergence and reduced settling times, particularly in scenarios that favor exploration or balanced optimization approach.
\begin{figure}[htb!]
    \centering
        \includegraphics[width=\linewidth]{Images/steady_state_error_low_res.png}
        \caption{Steady State Error KDE}
        \label{fig:steady_state_error_kdes}
\end{figure}

%In the balanced exploration-exploitation configuration shown in figure \ref{fig:steady_state_error_kdes} (left plot), the BO demonstrates a sharper and more concentrated density around a lower steady-state error, with its median error significantly closer to zero compared to DE's. This suggests that the BO is more effective at minimizing steady-state error when both exploration and exploitation are balanced. In the exploration-focused configuration (middle plot), the BO again shows a narrower distribution with a median error substantially below zero, indicating its superior performance in achieving more accurate PID tuning under conditions that favor exploration. In contrast, DE shows a wider and more dispersed distribution, reflecting less consistent performance. Under the exploitation-focused configuration (right plot), the KDE plots of both algorithms are more aligned, although the BO still maintains a slightly lower median steady-state error. Overall, these results suggest that the BO consistently provides lower steady-state errors across different configurations, particularly when exploration is emphasized, highlighting its robustness in the optimization task.
%\subsection{\rqfour{}} \label{rq4}
%\subsection{\rqfive{}} \label{rq5}

\subsection{Threats To Validity}
The primary threats to the validity of our trials and experiments concern the internal and external validity, as outlined below.

\begin{itemize}
\item{Internal Validity}
To address potential threats to internal validity due to confusion, we carefully selected the settings of the parameters for BO and DE. For BO, we used parameter values commonly used in search-based software engineering and optimization domains. Specifically,
the DE parameters were set using default values from the SciPy implementation \cite{2020SciPy}. Similarly, BO parameters followed the default settings from the Python Bayesian optimization implementation \cite{BO-library}, with exception specified in Section  \ref{sec:methodology}. Furthermore, DE and BO differ in their algorithmic nature and convergence mechanisms. To minimize bias, DE and BO were standardized in terms of initialization points, constraints, and stopping criteria. DE’s mutation strategies and BO’s acquisition function (using $\xi$ for exploration) were adjusted to align with the methodology described in Section \ref{sec:methodology}.
%DE is a population-based algorithm that creates solutions via mutation and crossover, with convergence mainly influenced by parameters like mutation rate and population size. BO, on the other hand, uses Gaussian processes to model the objective function, optimizing through an acquisition function that balances exploration and exploitation.
%, ensuring that comparisons reflected core performance characteristics rather than inherent algorithmic differences. 
\item{External Validity}
The choice of study subjects in our evaluation can influence the generalizability of the results. For this work, we used a robotic case study, specifically an industrial robotic system. Although this particular system has not been previously used in other studies, similar applications have been explored in the literature\cite{6-dof-arm-robot,alex_2021_dwmr,juraj_slovak__2018}. 

%\textcolor{orange}{Wu \& Chen studied the optimization of PID controller parameters for a 6-DOF robotic arm using Particle Swarm Optimization to enhance movement efficiency and smoothness \cite{6-dof-arm-robot}. Also, Štefek et al. proposed an optimization process for a fuzzy logic controller using a genetic algorithm to minimize energy consumption in a differential drive wheeled mobile robot \cite{alex_2021_dwmr}. Slovak et al. worked on the optimization of mobile robotic systems' trajectories using discrete Kalman filtration in indoor environments \cite{juraj_slovak__2018}.

Although our study focuses on a specific robotic system, we believe that our findings are generalizable to other cyber-physical systems (CPS), particularly in the robotics domain. Further experiments involving a broader class of CPS would enhance the applicability of our work. For practitioners in this field, our comparative study provides valuable insight into the performance trade-offs between BO and DE, and the selection of the best-suited optimizer for other applications. 
%BO’s faster convergence is beneficial in dynamic environments, while DE’s consistent performance makes it reliable when stability is critical. DE’s superior ability to avoid local optima makes it ideal for complex landscapes, while BO’s sensitivity to initial states calls for careful configuration. Understanding the exploration vs. exploitation trade-offs further helps tailor the optimization approach to specific system needs, enhancing overall performance.
%While the metrics we employed (e.g. ) are broadly applicable, we acknowledge that these metrics may not directly transfer to all CPS contexts, especially those involving distinct environments or simulation setups.
\end{itemize}




==> Sections/evaluation_extras.tex <==



Differential Evolution Results:

\begin{figure}
    \centering
    \includegraphics[width=0.90\linewidth]{Images/de_1.png}
    \caption{Experimentation Results DE - Initial State 1}
    \label{fig:DE_init_state_1}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.90\linewidth]{Images/de_2.png}
    \caption{Experimentation Results DE - Initial State 2}
    \label{fig:DE_init_state_2}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.90\linewidth]{Images/de_3.png}
    \caption{Experimentation Results DE - Initial State 3}
    \label{fig:DE_init_state_3}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.90\linewidth]{Images/de_4.png}
    \caption{Experimentation Results DE - Initial State 4}
    \label{fig:DE_init_state_4}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.90\linewidth]{Images/de_5.png}
    \caption{Experimentation Results DE - Initial State 5}
    \label{fig:DE_init_state_5}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.90\linewidth]{Images/de_6.png}
    \caption{Experimentation Results DE - Initial State 6}
    \label{fig:DE_init_state_6}
\end{figure}

%This figure below shows the best experiment for all 6:
\begin{figure}
    \centering
    \includegraphics[width=0.90\linewidth]{Images/de_best.png}
    \caption{Experimentation Results DE - Best of All}
    \label{fig:DE_init_state_6}
\end{figure}


%After running all six experiments on the DDMR designed for the task, these are the results' comparison:

\begin{table*}[t]
  \centering
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
  \hline
    Initial State & \# Trials & Settling Time (ms) & Rise Time (ms) & Overshoot (\%) & Total Time (s) & Steady-State Error (\%) & $K_p$ & $K_i$ & $K_d$ \\
    \hline
    1 & 11 & 2200 & 500 & 21.222 & 144 & 2.5 & 16.04974 &0.001 & 0.43061 \\
    2 & 41 & 2000 & 500 & 23.9 & 572 & 2.9222 & 15.60866 & 0.04862 & 0.70097 \\
    3 & 26 & 1600 & 900 & 10.3 & 358 & 0.4222 & 17.50521 & 0.02585 & 0.83124 \\
    4 & 11 & 2500 & 900 & 14.3 & 145 & 4.1111 & 21.00894 & 0.17 & 0.92844 \\
    5 & 21 & 1900 & 800 & 9.378 & 289 & 1.1778 & 15.54846 & 0.001 & 1.0 \\
    6 & 26 & 1700 & 900 & 11.711 & 361 & 0.7333 & 15.74136 & 0.05 & 0.08603 \\
    \hline
  \end{tabular}
  \caption{DE: Best result for each experiment}
  \label{table:DE-results}
\end{table*}


Trials were conducted to compare the performance of DE and BO. Table \ref{tab:trials-info} shows the initial gains ($K_p$, $K_i$, $K_d$) for each trial. The overshoot percentage and rise time constraints bounds are defined as in \ref{eq:overshootpercentagebounds} and \ref{eq:risetimebounds} respectively.
\begin{equation} \label{eq:overshootpercentagebounds}
Overshoot Percentage (\%): [0.0, 30.0] 
\end{equation}
\begin{equation} \label{eq:risetimebounds}
    Rise Time  (Sec): [0.0, 1.8]
\end{equation}


\begin{table}
    \centering
\caption{Trials information: ---}
\label{tab:trials-info}
    \begin{tabular}{|c|c|} \hline 
         Trial ID&  Initial $K_p$, $K_i$, $K_d$\\ \hline 
         1&  \\ \hline 
         2&  \\ \hline 
         3&  \\ \hline 
         4&  \\ \hline 
         5&  \\ \hline 
         6&  \\ \hline 
         7&  \\ \hline
    \end{tabular}
    
    
\end{table}

For the results in table \ref{table:balanced-exploration-exploitation} which represents the results for balanced exploration-exploitation experimentation. For time taken to converge for each experiment, it is seen that time taken by BO generally increases as the initial state changes from simpler controllers ($P$, $I$, $D$) to more complex ones ($PI$, $PD$, $PID$), for an example the time increases dramatically when moving from the $P$ controller (44 s) to the $PI$ controller (7396 s). Talking about DE, DE's time doesn't show a consistent pattern and is generally much lower than BO for complex controllers ($PI$, $PD$, $PID$). When talking about the number of iterations taken to converge, the number of iterations required by BO is generally lower compared to DE, BO typically requires fewer iterations as the controller complexity increases (with some exceptions like the $PI$ controller), DE requires significantly more iterations, especially noticeable in initial states 1 (126 iterations) and 5 (41 iterations). Regarding the settling time, BO tends to achieve a lower settling time compared to DE (1 tie, 3 for BO, and 2 DE), inducting that BO might lead to faster system response, and it's observed that the lowest settling time for BO is 1100 ms (initial state 3 - $PI$ controller), DE generally has higher settling times compared to BO. This suggests that DE might lead to slower system response. For steady-state Error comparison, BO achieves a steady-state error that is generally lower or comparable to DE, except for initial state 0 ($P$ controller), where BO has a higher error than DE. DE tends to produce steady states errors that are more consistent and generally positive, with fewer dramatic variations compared to BO. Finally, regarding gain parameters ($K_p$, $K_i$, $K_d$), BO tends to produce a lower (4 less, 1 almost equal and 1 more) $K_p$ value for most initial states compared to DE, which may result in less aggressive controller (may indicate a strong proportional control action), the $K_i$ values for BO are generally higher, especially for the $I$ controller (initial state 1), induction stronger integration action, the $K_d$ values for BO are lower or comparable to DE, which may lead to a less responsive derivative term. (quite varied, but BO tends to offer a more optimized derivation gain compared to DE in initial states 3 and 5). On the other hand, DE generally has a higher gain values across most controllers. $K_p$ values for DE are higher than BO, which may result in more aggressive controller. The $K_i$ values for DE are much lower, which may reduce the integral action's impact. $K_d$ values are higher or comparable to BO, which may lead to a more responsive derivative control.



Table \ref{table:exploration-focused} provides insights into the performance of BO and DE under an exploration-focused configuration. Firstly, the table shows that in this exploration-focused configuration, DE generally converges faster than BO, as evidenced by the shorter time and fewer iterations required in several initial states. For example, in initial state 0, DE converges in 146 seconds with 16 iterations, while BO takes 528 seconds and 28 iterations. This trend is also observed in initial state 3, where DE converges in 219 seconds compared to BO's 337 seconds. These observations suggest that DE is more efficient in this context, likely because it explores the parameter space more broadly and quickly identifies viable solutions.

However, the exploration focus of BO seems to impact its convergence in some states. For instance, BO fails to converge for initial states 1 and 5 reflecting potential difficulties in finding and optimal solution when initial conditions are less favorable or when the search space is particularly complex. DE, in contrast, successfully converges for all initial states, although it still requires significantly more time in initial state 5 (1363 seconds) to find a solution, indicating that both algorithms face challenges under certain conditions.

Furthermore, the differences in PID gain values between the algorithms illustrates how each optimizer navigates the parameter space. For example, in initial state 0, BO selects a proportional gain $K_p$ of 7.72, an integral gain $K_i$ of 0.0512, and a derivative gain $K_d$ of 0.5588, whereas DE opts for higher $K_p$ and $K_d$ values (12.5 and 0.635 respectively) with much lower $K_i$ (0.001). These variations suggest that DE may prioritize minimizing the steady-state error (-3.36 degrees for DE vs. 2.76 degrees for BO) by choosing a higher proportional gain, even at the expense of slightly more aggressive control actions. On the other hand, BO's choice of a relatively higher $K_i$ indicates an attempt to better handle steady-state errors, although it may lead to longer settling times.


Table \ref{table:exploitation-focused} presents the results of PID auto-tuning under an exploitation-focused configuration for BO and DE.

Under the exploitation-focused approach, DE consistently demonstrates superior convergence ability compared to BO. In several initial states, BO fails to converge, such as in initial states 0 and 5. Conversely, DE successfully converges across all initial states, albeit sometimes requiring significant time and iterations. For example, in initial state 5, DE converges in 1276 seconds over 91 iterations, while BO does not converge. This pattern suggests that DE's strategy pf systematically exploiting the parameter space is more effective for reaching a solution when there is less emphasis on exploration and more on refining known good solutions.

Additionally, the results highlight differences in the PID gain adjustments made by each optimizer. For instance, in initial state 2, BO converges with a high proportional gain ($K_p = 22.98$) and integral gain ($K_i = 0.92$), indicating a more aggressive control strategy likely aimed at reducing steady-state errors quickly. However, this strategy does not always result in a lower steady-state error, as seen by the relatively high error of 15.52 degrees for DE, which adopts a lower $K_i$ of 0.001 but with a slightly more balanced approach using a moderate $K_p$ of 20.0. This indicates that while BO may attempt to leverage more aggressive gains, DE achieves more consistent results by balancing the gains more conservatively.





\begin{table*}[t]
  \centering
  \caption{Exploration Focused}
  \label{table:exploration-focused}
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
  \hline
    Initial State& Optimizer& Time (s)& \# Iterations&  Settling Time (ms)&Steady State Error (deg)&$K_p$ & $K_i$&$K_d$\\
    \hline
    \multirow{2}{*}{0}& BO& 528& 28 & 1800 & 2.76& 7.716153 & 0.051234 & 0.55882\\
    & DE& 146& 16 & 1800 & -3.36& 12.5& 0.001& 0.635\\ \hline 
    \multirow{2}{*}{1}& BO& didn't converge & 150 & -& -& -& -& -\\
    & DE& 146& 11 & 2200 & 8.53& 12.0& 0.0& 0.78\\ \hline 
    \multirow{2}{*}{2}& BO& 72& 5 & 1300 & 0.48& 1.628304 & 0.596086 & 0.67511\\
    & DE& 145& 11 & 1400 & 12.35& 8.0& 0.0& 0.59\\\hline
    \multirow{2}{*}{3}& BO& 337& 22 & 1700 & -3.42& 5.192586 & 0.000171 & 0.034392 \\
    & DE& 219& 21 & 1500 & 2.24& 9.556112 & 0.042521 & 0.45975\\ \hline
    \multirow{2}{*}{4}& BO&330& 22 & 1700 & -2.41& 6.639665 & 0.019850 & 0.658243 \\
    & DE& 420& 31 & 2400 & 1.08& 15.6875& 0.08216& 0.712342 \\ \hline
    \multirow{2}{*}{5}& BO& didn't converge & 150 & -& -& -& -& -\\
    & DE& 1363& 111 & 2500 & 4.45& 18.542969 & 0.334112 & 0.818519 \\ \hline
  \end{tabular}
\end{table*}

\begin{table*}[t]
  \centering
  \caption{Exploitation Focused}
  \label{table:exploitation-focused}
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
  \hline
    Initial State& Optimizer& Time (s)& \# Iterations&  Settling Time (ms)&Steady State Error (deg)&$K_p$ & $K_i$&$K_d$\\
    \hline
    \multirow{2}{*}{0}& BO& didn't converge & 150 & -& -& -& -& -\\
    & DE& 147& 16 & 1700 & -1.72& 8.193706 & 0.001& 0.001\\ \hline 
    \multirow{2}{*}{1}& BO& 185& 13 & 1600 & 2.28& 6.511244 & 0.085351 & 0.436861 \\
    & DE& 1236& 91 & 1900 & 2.33& 12.497146 & 0.165878 & 0.952479 \\ \hline 
    \multirow{2}{*}{2}& BO& 3287& 70 & 2300 & -2.1& 22.981145 & 0.924054 & 0.306222 \\
    & DE& 144& 16 & 2500 & 15.52& 20.0& 0.001& 1.0\\\hline
 \multirow{2}{*}{3}& BO& 386& 24 & 1400 & 3.72& 4.658873 & 0.048825 & 0.477699 \\
 & DE& 975& 71 & 2400 & 2.26& 18.292283 & 0.262592 & 0.894938 \\ \hline
 \multirow{2}{*}{4}& BO&242& 17 & 2100 & 3.61& 12.24331& 0.173875 & 0.763353 \\
 & DE& 218& 16 & 1600 & 4.46& 4.208397 & 0.001& 1.0\\ \hline
 \multirow{2}{*}{5}& BO& didn't converge & 150 & -& -& -& -& -\\
 & DE& 1276& 91 & 2400 & 6.57& 12.911706 & 0.003338 & 0.091413 \\ \hline
  \end{tabular}
\end{table*}
